Making Weak Memory Models Fair

Liveness properties, such as termination, of even the simplest shared-memory concurrent programs under sequential consistency typically require some fairness assumptions about the scheduler. Under weak memory models, we observe that the standard notions of thread fairness are insufficient, and an additional fairness property, which we call memory fairness, is needed. In this paper, we propose a uniform definition for memory fairness that can be integrated into any declarative memory model enforcing acyclicity of the union of the program order and the reads-from relation. For the well-known models, SC, x86-TSO, RA, and StrongCOH, that have equivalent operational and declarative presentations, we show that our declarative memory fairness condition is equivalent to an intuitive model-specific operational notion of memory fairness, which requires the memory system to fairly execute its internal propagation steps. Our fairness condition preserves the correctness of local transformations and the compilation scheme from RC11 to x86-TSO, and also enables the first formal proofs of termination of mutual exclusion lock implementations under declarative weak memory models.

==> mcslock.tex <==
\section{MCS Lock}
\label{sec:mcslock}

Consider the following implementation of the lock passing mechanism of the MCS lock (simplified for clarity):
  $$\inarrT{
    \assignInst{\kw{int}^* \; locked}{\kw{new}\; \kw{int}(0)} \\
    \assignInst{\kw{int}^{**} \; next}{\kw{new}\; \kw{int}^*(\kw{null})} \\
    \funcDecl{\kw{void}}{receiveLock}{}{
      \kw{int}\; r \\
      \writeInst{[locked]}{1} \\
      \writeInst{[next]}{locked}\\
      \repeatInst{ \readInst{r}{[locked]} }{(r\; = \; 0)}
    }
    \funcDecl{\kw{void}}{passLock}{}{
      \kw{int}^*\; l \\
      \repeatInst{ \readInst{l}{[next]} }{(l\; \not = \; \kw{null})} \\
      \writeInst{[l]}{0}
    }
  }$$

We verify that the lock passing can not get stuck, i.e., spinloops terminate in the following client which passes the lock from the current owner to the next:
\begin{equation*}
\tag{MCS-Client}\label{ex:MCS-client}
\inarrII{
  passLock()
}{
  receiveLock()
}
\end{equation*}
\begin{theorem}
\ref{ex:MCS-client}'s thread-fair behaviors
under $G^\fair_{\set{\SC, \TSO, \RA}}$ are all finite.
\end{theorem}
\begin{proof}
Observe that the $\lMO$-maximal store on $\mathit{next}$ sets $[\mathit{next}] = \mathit{locked}$.
Thus by \cref{thm:spinloop termination basic}, the spinloop in $\mathit{passLock}$ terminates. 
Observe that it only terminates after reading from that store.
Thus after termination we have $\mathit{l} = \mathit{locked}$.
Due to thread-fairness, the passing thread executes a store $w$ setting $[\mathit{l}]$ to $0$, and this store appears in the $\lMO$ of $[\mathit{l}]=[\mathit{locked}]$.
To show that the spinloop in $\mathit{receiveLock}$ terminates, it suffices (with \cref{thm:spinloop termination basic}) to show that $w$ is $\lMO$-maximal. 
We show the proof only for $\RA$ since it allows the most behaviors.
Consider for the sake of contradiction the following (partially depicted) execution graph, which depicts the only legal $\lMO$ in which $w$ is not $\lMO$-maximal:
\begin{equation*}
\small
\begin{tikzpicture}[yscale=1,xscale=1.5]
  \node (0x)  at (-1,2) {$\evlab{\lW}{}{[\mathit{locked}]}{0}$};
  \node (0y)  at (1,2) {$\evlab{\lW}{}{[\mathit{next}]}{\kw{null}}$};
  \node (12)  at (-1,1) {$\evlab{\lW}{}{[\mathit{locked}]}{1}$ };
  \node (13)  at (-1,0) {$\evlab{\lW}{}{[\mathit{next}]}{\mathit{locked}}$ };
  \node (21)  at (1,1) {$\evlab{\lR}{}{[\mathit{next}]}{\mathit{locked}}$ };
  \node (22)  at (1,0) {$w: \evlab{\lW}{}{[\mathit{locked}]}{0}$ };
  \draw[po] (0x) edge (12) edge (21);
  \draw[po] (0y) edge (21) edge (12);
  \draw[po] (12) edge (13);
  \draw[po] (21) edge (22);
      \draw[rf] (13) edge node[below] {\smaller$\lRF$} (21);
  \draw[mo,bend right=15] (22) edge node[above] {$\lMO$} (12);
\end{tikzpicture}
\end{equation*}
which has a $\lRA_{\lLOC}$-cycle and is therefore not $\G_\RA$-consistent.%
\end{proof}
Note that $w$ is only $\lMO$-maximal because $\lRA_{\lLOC}$ is irreflexive in $\G_{\set{\RA,\SC,\TSO}}$.
In other memory systems (e.g., ARMv8, PowerPC, (R)C11), $w$ is not guaranteed to be $\lMO$-maximal without additional fences, and locks that pass ownership in this manner will not always terminate even in thread\&memory-fair executions.
This includes the HMCS lock, for which ``the fences necessary for the HMCS lock on systems with processors that use weak ordering'' suggested in the original paper~\cite[p.~218]{hmcs} do not ensure termination on any of these systems.
Indeed we have reproduced this non-terminating behavior on an ARMv8 server with 128 cores using the fences suggested in that paper, resulting eventually in a system-wide, permanent hang.
This shows that termination of spinloops under weak memory models is a practically important topic which has so far been mostly ignored in the literature.

